Topological Causal Effects

Estimating causal effects is particularly challenging when outcomes arise in complex, non-Euclidean spaces, where conventional methods often fail to capture meaningful structural variation. We develop a framework for topological causal inference that defines treatment effects through differences in the topological structure of potential outcomes, summarized by power-weighted silhouette functions of persistence diagrams. We develop an efficient, doubly robust estimator in a fully nonparametric model, establish functional weak convergence, and construct a formal test of the null hypothesis of no topological effect. Empirical studies illustrate that the proposed method reliably quantifies topological treatment effects across diverse complex outcome types.

==> main_summary.tex <==
Modern scientific questions often demand causal inference methods that go beyond scalar summaries such as means or variances. 
In many complex systems, interventions produce structural or geometric changes in the data that cannot be captured by traditional estimands. 
For example, a medical treatment may trigger the formation of additional molecular loops, a new neural connection may appear in brain connectivity networks, or an economic intervention might alter the connectivity pattern in a financial network. 
These structural shifts are topological in nature and are invisible to conventional estimators of average treatment effects. 
Our work fills this methodological gap by developing a rigorous framework for \emph{topological causal inference}.

\medskip
\noindent
\textbf{Motivation.} 
Topological Data Analysis (TDA) provides a principled way to capture such structural changes by representing data in terms of homological features such as connected components, cycles, and voids. 
For a given outcome $Y$, we first construct a filtration $\F$ (e.g., via Vietoris–Rips or sublevel-set filtration), yielding a persistence diagram $\D_d(\F)$ that records the birth and death times of all $d$-dimensional homological features. 
However, persistence diagrams are multisets and not directly amenable to statistical operations. 
To make them suitable for estimation and inference, we map them into the space of functions via the \emph{power-weighted silhouette transform}:
\[
\phi(t; \D_d) 
= \frac{\sum_{p \in \D_d} |b_p - a_p|^{r} \Lambda_p(t)}
{\sum_{p \in \D_d} |b_p - a_p|^{r}}, 
\qquad t \in \mathbb{T},
\]
where $p = (a_p, b_p)$ is a birth–death pair, $\Lambda_p(t)$ is its associated triangular “tent function,” and $r>0$ weights features according to their persistence. 
This functional summary is 1-Lipschitz and lies in a separable Hilbert space, enabling the application of empirical process tools.

\medskip
\noindent
\textbf{Topological Causal Effect.}
Let $Y^{a}$ denote the potential outcome under treatment $a \in \{0,1\}$, and let $\D_d^{a}$ be the corresponding persistence diagram for homology dimension $d$. 
We define the \emph{topological causal effect} as the functional contrast
\[
\psi_d(t) = 
\E\!\Big[\phi^{1}(t; \D_d^{1}) - \phi^{0}(t; \D_d^{0})\Big],
\qquad t \in \mathbb{T},
\]
where $t \mapsto \psi_d(t)$ characterizes how the intervention affects the strength of $d$-dimensional features across scales. 
A positive $\psi_d(t)$ indicates the creation or strengthening of topological features, while negative values indicate their disappearance. 
This functional representation preserves scale information, is robust to noise, and allows us to analyze topological changes at multiple resolutions simultaneously.

\medskip
\noindent
\textbf{Methodology.}
Given observed data $\{(X_i, A_i, Y_i)\}_{i=1}^n$, we propose a semiparametric estimator for $\psi_d(t)$ based on its efficient influence function (EIF):
\[
\varphi(t, Z; \eta)
= \mu_1(t, X) - \mu_0(t, X) + 
\left(\frac{A}{\pi(X)} - \frac{1-A}{1-\pi(X)}\right)
\Big[\phi(t; \D_d) - \mu_A(t, X)\Big],
\]
where $\pi(X)=\P(A=1 \mid X)$ is the propensity score, $\mu_a(t,X)=\E[\phi(t;\D_d) \mid X,A=a]$ is the silhouette regression function, and $\eta = (\pi,\mu_0,\mu_1)$ denotes the nuisance parameters. 
The proposed \emph{augmented inverse probability weighted (AIPW)} estimator is
\[
\widehat{\psi}_{AIPW}(t) = 
\Pn\!\big[\varphi(t, Z; \widehat{\eta})\big],
\]
which is $\sqrt{n}$-consistent and asymptotically Gaussian under standard conditions, even with flexible, nonparametric nuisance estimators. 
By leveraging new stability bounds for weighted silhouettes, we establish weak convergence of $\widehat{\psi}_{AIPW}(t)$ in $\ell^{\infty}(\mathbb{T})$, enabling the construction of uniform confidence bands. 
This also allows us to formulate a formal hypothesis test for the null of no topological effect, 
\[
H_0: W_1(\D^1,\D^0)=0,
\]
where $W_1$ is the $1$-Wasserstein distance between persistence diagrams. 

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{0.455\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/running_protein.png}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.525\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/running_pd.png}
    \end{minipage}
    \caption{Left: Example of untreated vs.\ treated macromolecule structures. 
Right: Corresponding persistence diagrams, highlighting treatment-induced changes in first-order homology features.}
    \label{fig:running_example}
\end{figure}

Figure~\ref{fig:running_example} illustrates the intuition: treatment induces new cycles in the molecular graph that are captured as additional points away from the diagonal in the persistence diagram. 
Our framework converts these structural differences into a well-defined causal estimand, allowing for formal statistical testing and robust inference.

\medskip
\noindent
\textbf{Potential Applications.} 
This framework applies broadly to scientific domains where outcomes exhibit rich topological structure: neuroscience (stimulus-driven changes in brain connectivity networks), computational biology (protein folding under mutations or drugs), climate science (evolution of spatio-temporal patterns), finance (shifts in correlation networks under interventions), and dynamical systems (detecting regime shifts). 
By providing a statistically rigorous, scalable, and general-purpose approach to quantifying structural causal effects, our method opens the door to a new class of causal analyses that are sensitive to global and local topology alike.
